Boosting Meta-Training with Base Class Information for Few-Shot Learning

Few-shot learning, a challenging task in machine learning, aims to learn a classifier adaptable to recognize new, unseen classes with limited labeled examples. Meta-learning has emerged as a prominent framework for few-shot learning. Its training framework is originally a task-level learning method, such as Model-Agnostic Meta-Learning (MAML) and Prototypical Networks. And a recently proposed training paradigm called Meta-Baseline, which consists of sequential pre-training and meta-training stages, gains state-of-the-art performance. However, as a non-end-to-end training method, indicating the meta-training stage can only begin after the completion of pre-training, Meta-Baseline suffers from higher training cost and suboptimal performance due to the inherent conflicts of the two training stages. To address these limitations, we propose an end-to-end training paradigm consisting of two alternative loops. In the outer loop, we calculate cross entropy loss on the entire training set while updating only the final linear layer. In the inner loop, we employ the original meta-learning training mode to calculate the loss and incorporate gradients from the outer loss to guide the parameter updates. This training paradigm not only converges quickly but also outperforms existing baselines, indicating that information from the overall training set and the meta-learning training paradigm could mutually reinforce one another. Moreover, being model-agnostic, our framework achieves significant performance gains, surpassing the baseline systems by approximate 1%.

==> 04MethodOld.tex <==
In this section, we first provide our motivation %in Section \ref{section_4_1} 
and then introduce our Boost-MT method. % in Section \ref{section_4_2}.

\subsection{Motivation}
\label{section_4_1}
Many prior works~\cite{goodembedd, Meta-Baseline} have demonstrated that few-shot classifiers benefit significantly from non-episodic pre-training. Therefore, when the meta-training %is continued based on 
continues to base on 
the pre-training, the model performance should continue to improve until converging.  %stably. 
%%-------------------------------------------------
% \begin{figure*}
% \centering
% \subfloat[]{\includegraphics[width=0.3\linewidth]{vctor-1.pdf}%
% \label{fig_sub1}
% }
% \hfil
% \subfloat[]{\includegraphics[width=0.28\linewidth]{vctor-2.pdf}%
% \label{fig_sub2}}
% \hfil
% \subfloat[]{\includegraphics[width=0.3\linewidth]{vctor-3.pdf}%
% \label{fig_sub3}}

% \caption{Illustration of the relationship between distance $d_{meta}$ and distance $d_{true}$. $d_{meta}$ represents the distance between representations obtained through training, and $d_{true}$ represents the true distance between two representations, which can be represented by the combination of $d_{cos}$ and $d_{unknown}$. After the pre-training, the relationship between $d_{meta}$ and $d_{true}$ is as shown in %Figure \ref{fig:sub1}
% (a); As the meta-training proceeds, $d_{meta}$ gradually approaches $d_{cos}$ and $d_{true}$, as shown in %Figure \ref{fig:sub2}
% (b), which will improve the model performance; As the training continues, as shown in %Figure \ref{fig:sub3}
% (c), $d_{meta}$ continues to approach $d_{cos}$, but it deviates from $d_{true}$, leading to a decline on the model performance. Note that here we only use two-dimensional coordinates to illustrate the relative relationship between distances.}
% \label{fig_short}
% \end{figure*}
\begin{figure*}
\centering
\subfloat[$mini$Imagenet]{
\begin{tikzpicture}[scale=0.8] %tikz图片

          \begin{axis}[
            xlabel=Epoch, %横坐标名
            % \vspace{3mm}
            ylabel=Accuracy $(\%)$, %纵坐标名
            tick align=inside, %刻度在外显式
            legend style={at={(0.65,0.9))},anchor=north} %图例在图下方显示  0.88
            ]
        
        %第一条线，mark是折线标示形状
          \addplot[smooth,red, line width = 1.5pt] plot coordinates { 
            (0,88.44)
            (5,87.72)
            (10,86.93)
            (15,86.10)
            (20,84.66)
            (25,83.61)
            (30,82.64)
            (40,80.61)
            (50,78.12)
            (60,76.33)
            (70,75.34)
            (80,73.20)
            (90,71.22)
            (100,70.83)
        
        };
          \addlegendentry{conventional classification}
        
          \addplot[smooth,blue, line width = 1.5pt] plot coordinates { 
            (0,77.76)
            (5,79.16)
            (10,79.26)
            (20,79.00)
            (30,78.75)
            (40,78.57)
            (50,78.22)
            (60,77.82)
            (70,77.40)
            (80,77.00)
            (90,76.60)
            (100,76.15)
        
        };
          \addlegendentry{few-shot classification}
        
          \end{axis}
\end{tikzpicture}
\label{fig:sub1}}
\hfil
\subfloat[$tiered$Imagenet]{
\begin{tikzpicture}[scale=0.8] %tikz图片

      \begin{axis}[
            xlabel=Epoch, %横坐标名
            % \vspace{3mm}
            ylabel=Accuracy $(\%)$, %纵坐标名
            tick align=inside, %刻度在外显式
            legend style={at={(0.65,0.90))},anchor=north} %图例在图下方显示
            ]
        
        %第一条线，mark是折线标示形状
      %第二条线，mark是折线标示形状
        \addplot[smooth,red, line width = 1.5pt] plot coordinates { 
            (0,77.33)
            (5,74.78)
            (10,73.18)
            (20,70.85)
            (30,68.23)
            (40,65.71)
            (50,61.80)
            (60,59.71)
            (70,57.34)
            (80,55.04)
            (90,60.48)
            (100,60.39)
        
        };
          \addlegendentry{conventional classification}
        \addplot[smooth,blue, line width = 1.5pt] plot coordinates { 
            (0,83.34)
            (5,82.09)
            (10,80.62)
            (20,78.09)
            (30,76.96)
            (40,75.75)
            (50,75.03)
            (60,74.03)
            (70,72.76)
            (80,72.81)
            (90,72.22)
            (100,71.54)
        
        };
          \addlegendentry{few-shot classification}
        
      \end{axis}
\end{tikzpicture} 
\label{fig:sub2}}
\caption{Accuracy of the conventional classification and few-shot classification during meta-training.
   (a) Accuracy of the second stage of Meta-Baseline on $mini$ImageNet along with the training process;
   and (b) accuracy  the second stage of Meta-Baseline on $tiered$ImageNet along with the training process. The few-shot task is set to 5 way 5 shot.}
\label{fig:conventional}
\end{figure*}
%-----------------------------------------------------------------
%-----------------------------------------------------
However, as shown in Figure \ref{fig:dif-measure}, we observe that in the second stage of Meta-Baseline, the performance on the validation set first increases, then 
declines, and finally, is even lower than that of the Prototypical Networks.
It seems that the pre-training restricts the meta-learning to further improve the model performance.
% We speculate that the cosine similarity metric used in the second stage may not effectively capture the representation information learned in the pre-training stage.

% To test this hypothesis,  
In order to investigate whether this phenomenon is associated with the metric method, we conduct experiments using Euclidean distance or a combination of cosine similarity and Euclidean distance instead of the cosine similarity alone. 
Interestingly, we find that only using Euclidean distance %decreases the performance and also results in slower attenuation.
will decrease the performance but also result in slower decays. %attenuation.
We further validate the Manhattan distance and Chebyshev distance and come up with the similar phenomenon.

% 2023-08-13--------------------------
%We attempted to 
% We try to provide an explanation for this phenomenon based on the assumption presented in Figure \ref{fig_short}. In few-shot classification, the first step is to map the image to the embedding
% space and determine which support class the query is closest to by measuring the distance in between. The embedding space is a high-dimensional space where the distance between any two vectors (referred to as the true distance) can be theoretically measured. However, obtaining the true distance is challenging in practice. Hence, we make the assumption that there exists a true distance, denoted as $d_{true}$.
% Although it is not possible to directly measure the complete
% theoretical distance, we can partially capture it using certain metrics such as cosine similarity, represented as $d_{cos}$.
% The remaining portion cannot be measured is denoted as
% $d_{unknown}$. Here we only employ two-dimensional coordinates to illustrate the relative relationships between distances.
% %---------------------------------------------------
% % As illustrated in Figure \ref{fig:short}, we assume that the distance of true representations ($d_{true}$) can be measured using cosine similarity ($d_{cos}$) and some additional measurement distance that is unknown ($d_{unknown}$).
% The distance $d_{meta}$ in Figure \ref{fig_sub1} indicates the representation distance obtained through the first stage. 
% As shown in Figure \ref{fig_sub2}, during the course of the second stage under the cosine similarity metric learning, %measurement,
% $d_{meta}$ gradually approaches $d_{cos}$ and the ground-truth $d_{true}$, resulting in performance improvement and explaining the phase $a \to b$ in Figure \ref{fig:dif-measure}.

% However, as shown in Figure \ref{fig_sub3}, $d_{meta}$ continues to approach $d_{cos}$ as the training continues and deviates from the ground-truth $d_{true}$, leading to performance degradation and explaining the phase after point $b$ in Figure \ref{fig:dif-measure}.
% Moreover, the representation from the first stage can even have a negative impact on meta-training, resulting in inferior performance compared to the Prototypical Networks, as shown in the phase after point $c$ in Figure \ref{fig:dif-measure}.

% Although a theoretical method exist to measure the %fixed 
% latent representation, it is not practically obtainable. If the measurement is not chosen correctly, it can have a negative impact on meta-training.
% Therefore, utilizing a fixed embedding space obtained through pre-training is challenging.

To investigate the underlying factors behind this phenomenon, we conduct a series of experiments. In the meta-training phase, we not only assess the feature extractor's classification proficiency on few-shot tasks but also utilize both the feature extractor and classification header trained in the first stage to carry out conventional classification tasks based on base classes. The results are illustrated in Figure \ref{fig:conventional}. We observed that during the second stage, there is an initial improvement in the model's performance for few-shot classification tasks; however, it gradually deteriorates thereafter. Furthermore, there is a consistent decline in the model's performance for conventional classification tasks, indicating that second-stage meta-learning hampers the model's ability to transfer knowledge across different classes. Consequently, we hypothesize that maintaining the model's conventional classification capability during the second stage could potentially enhance its overall performance.


% \HK{Why the above analysis is related to our method?} 

%Inspired by SVRG, 
Thereby, we propose a novel framework termed Boost-MT that leverages the information from the base class to guide meta-learning instead of relying on direct pre-training. 

\subsection{Boosting meta-training with base class information}
\label{section_3_4}
As shown in Figure \ref{fig:framwork}, our method consists of %outer loop and inner loop. 
two loops. The outer loop is executed $S$ times in one epoch, and each outer loop corresponds to $T$ inner loops. The network model consists of a feature extractor $f_\theta$ used in both outer loop and inner loop, a classification header $fc_\omega$ used in outer loop, and a cosine similarity measurement function $d(\cdot,\cdot)$ used in inner loop. Here we randomly initialize $f_\theta$ and $fc_\omega$.

\begin{figure*}
\begin{center}
  \includegraphics[width=0.9\linewidth]{svrg_0925.pdf} 
\end{center}
   \caption{The main framework of our model. In the outer loop, we calculate the classification loss of one large batch from base classes and only update the linear classifier. In the inner loop, we use the meta-learning method to calculate the loss of tasks and update the model by inner loss and outer loss. %When the inner loop is completed, it re-enters the outer loop.
   The two loops are executed alternately, with $T$ inner loops per one outer loop. }
\label{fig:framwork}
\end{figure*}

In each outer loop, we first randomly sample a large set $\mathcal{D}^{out}$ with $N_b$ images from $D^{base}$. Then we calculate the loss $\Tilde{\mu}$ of $D^{out}$ by \eqref{e3} and only update $fc_{\omega}$. 
When all outer loops in one epoch are done, all samples in  $\mathcal{D}^{base}$ are traversed once.
Before the first inner loop begins, we randomly sample $T$ tasks $\mathcal{T} = {\{ (\mathcal{D}_t^{spt}, \mathcal{D}_t^{qry}) \}}_{t=1}^T$ from $\mathcal{D}^{base}$ as standard few-shot learning.

% \begin{align}\label{e3}
%     \Tilde{\mu} = \frac{1}{N_b}\sum_{(\mathbf{x},y) \in \mathcal{D}^{out}}\mathcal{L}(fc_{\Tilde{\omega}_{s-1}}(f_{\Tilde{\theta}_{s-1}}(\mathbf{x})),y),
% \end{align}
\begin{align}\label{e3}
    \Tilde{\mu} = \frac{1}{N_b}\sum_{(\mathbf{x},y) \in \mathcal{D}^{out}}\mathcal{L}_{\mathbf{x}}(f_{\Tilde{\theta}_{s-1}},fc_{\Tilde{\omega}_{s-1}}),
\end{align}
where $s=\left\{1,...,S\right\}$, and $S$ is the number of outer loops. $\Tilde{\theta}_{s}$ and $\Tilde{\omega}_{s}$ represent the parameters of $f_{\theta}$ and $fc_{\omega}$ in the $s$-th iteration of outer loop, respectively.

In each inner loop, one task is calculated at a time. The feature extractor $f_{\theta}$ extracts the embedded representations of the support set and query set. We calculate the prototype of each class in the support set by \eqref{e1}. 
For each sample in the query set, we use cosine similarity measurement $d(\cdot,\cdot)$ and predict its label by \eqref{e2}.
The loss of query point $\mathbf{x}$ is calculated by the cross entropy loss.
The inner loss of the query set $\sigma$ is calculated by $f_{\theta}$ with inner loop parameters and cosine similarity measurement $d(\cdot,\cdot)$, as in \eqref{e4}.
% The outer-loss of query set is calculated by $f$ and $g$ with outer loop parameters.
The outer loss of the query set $\Tilde{\sigma}$ is calculated by $f_{\theta}$ with outer loop parameters and $d(\cdot,\cdot)$, as in \eqref{e5}.
The inner and outer losses of the query set and the outer loss of $\mathcal{D}^{out}$ will both be used to update the parameters of $f_{\theta}$, as in \eqref{e6}.
In the next inner loop, the updated parameters in the 
previous inner loop are used to calculate inner-loss until all inner loops are done.
%When all the inner loops are done,
Then, the parameters of $f_\theta$ in the next outer loop are inherited from the previous inner loop.
The details are shown in Algorithm \ref{alo1}.

% \begin{align}\label{e4}
%     \sigma = \frac{1}{NQ}\sum_{(\mathbf{x},y) \in \mathcal{D}_t^{qry}}\mathcal{L}(p_{\theta_{t-1}}(y=n|\mathbf{x}),y),
% \end{align}
% \begin{align}\label{e5}
%     \Tilde{\sigma} = \frac{1}{NQ}\sum_{(\mathbf{x},y) \in \mathcal{D}_t^{qry}}\mathcal{L}(p_{\Tilde{\theta}_{s-1}}(y=n|\mathbf{x}),y)
% \end{align}
\begin{align}\label{e4}
    \sigma = \frac{1}{NQ}\sum_{(\mathbf{x},y) \in \mathcal{D}_t^{qry}}\mathcal{L}_{\mathbf{x}}(f_{\theta_{t-1}},d(\cdot,\cdot)),
\end{align}
where $t=\left\{1,...,T\right\}$, and $T$ is the number of inner loops. ${\theta}_{t}$ represents the parameters of $f_{\theta}$ in the $t$-th iteration of inner loop.
\begin{align}\label{e5}
    \Tilde{\sigma} = \frac{1}{NQ}\sum_{(\mathbf{x},y) \in \mathcal{D}_t^{qry}}\mathcal{L}_{\mathbf{x}}(f_{\Tilde{\theta}_{s-1}},d(\cdot,\cdot)),
\end{align}
\begin{align}\label{e6}
    \theta_t = \theta_{t-1} - \beta(\nabla\sigma - \nabla\Tilde{\sigma} + \nabla\Tilde{\mu}) .
\end{align}

As analyzed in Section \ref{section_1}, a fixed embedding space from pre-training is difficult to exploit for meta-training.
Unlike the meta-learning method with pre-training, although we calculate the loss on the base classes in the outer loop, we do not update parameters of the feature extractor, avoiding the direct update of representation information by $\mathcal{D}^{base}$. 

The key aspect of our method is that the loss function is updated using the loss in each task during the inner loop of updating the feature extractor, which simultaneously draws the feature extractor in the outer loop and the last update.
Instead of continuing the meta-learning on the already convergent classification feature extractor, we use the gradient generated by classification training to correct the optimization direction of the meta-learning, so as to provide guidance during each meta-training, which not only can inherit the class transfer ability brought by classification training, but also can better adapt to the task of meta-learning.
Therefore, our end-to-end method can still utilize the information from $\mathcal{D}^{base}$ by updating inner parameters through outer loss and inner loss, which avoids mutual subtraction between the two stages and boosts meta-training.

%---------------------------
\begin{algorithm}[t]
\caption{The Boost-MT Method}\label{alg:alo1}
\begin{algorithmic}[1]
\STATE \textbf{Input:} 
%\hspace*{0.02in} {\bf Require:}  
base classes $\mathcal{D}^{base}$,
%\hspace*{0.02in} {\bf Require:}  
feature extractor with parameters $\theta$: $f_{\theta}$,
%\hspace*{0.02in} {\bf Require:}  
classification header with parameters $\omega$: $fc_{\omega}$,
%\hspace*{0.02in} {\bf Require:} 
hyperparameters on step size: $\alpha, \beta$ 
%\hspace*{0.02in} {\bf Require:}  
%RandSample($\mathcal{D},N$): randomly sample $N$ images from $\mathcal{D}$\\
%\hspace*{0.02in} {\bf Require:} 
%$d(\cdot,\cdot)$: calculate the cosine similarity between two vectors\\
%\hspace*{0.02in} {\bf Require:} 
%$\mathcal{L}$: cross entropy loss
% \STATE \textbf{Output:} $\Tilde{\theta}_S$
\STATE \textbf{Output:} $\theta$
\STATE \textbf{Require:} RandSample($\mathcal{D},N$): randomly sample $N$ images from $\mathcal{D}$ 
\STATE Initialize $\Tilde{\theta}_0, \Tilde{\omega}_0$
\FOR{$s=1,2,3, \dots,S$}
    \STATE $\mathcal{D}^{out} \leftarrow$ RandSample$(\mathcal{D}^{base}, N_b)$
    % \State $\Tilde{\mu} = \frac{1}{N_b}\sum_{(\mathbf{x},y) \in \mathcal{D}^{out}}\mathcal{L}_{\mathbf{x}}(f_{\Tilde{\theta}_{s-1}},g_{\Tilde{\omega}_{s-1}})$
    \STATE Compute the loss of $\mathcal{D}^{out}$ by \eqref{e3}
    \STATE $\Tilde{w}_s = \Tilde{w}_{s-1} - \alpha\nabla\Tilde{\mu}$
    \STATE $\theta_{0}=\Tilde{\theta}_{s-1}$
    \STATE Sample $\mathcal{T} = {\{ (\mathcal{D}_t^{spt}, \mathcal{D}_t^{qry}) 
    \}}_{t=1}^T$ from $\mathcal{D}^{base}$
    \FOR{$t=1,2,3,\dots,T$}
       % \State $\sigma = \frac{1}{NQ}\sum_{(\mathbf{x},y) \in \mathcal{D}_t^{qry}}\mathcal{L}_{\mathbf{x}}(f_{\theta_{t-1}},d(\cdot,\cdot))$ 
       %  \State $\Tilde{\sigma} = \frac{1}{NQ}\sum_{(\mathbf{x},y) \in \mathcal{D}_t^{qry}}\mathcal{L}_{\mathbf{x}}(f_{\Tilde{\theta}_{s-1}},d(\cdot,\cdot))$
       %  \State $\theta_t = \theta_{t-1} - \beta(\nabla\sigma - \nabla\Tilde{\sigma} + \nabla\Tilde{\mu}) $
        \STATE Compute the prototype of the $t$ task by \eqref{e1}
        \STATE Compute the probability of the query point $\mathbf{x}$ by \eqref{e2}
        \STATE Compute the inner loss of $\mathcal{D}_t^{qry}$ with inner loop parameters by \eqref{e4}
        \STATE Compute the outer loss of $\mathcal{D}_t^{qry}$ with outer loop parameters by \eqref{e5}
        \STATE Update $\theta$ based on \eqref{e6}
    \ENDFOR
    % \State \textbf{option I:}  
    \STATE $ \Tilde{\theta}_s = \theta_T$
    % \State \textbf{option II:}$\ \Tilde{\theta}_s = \theta_t$ from randomly chosen $t \in (1,2,3,\dots,T)$
\ENDFOR
\STATE $ \theta = \Tilde{\theta}_S$
\STATE \textbf{return}  $\theta$
\end{algorithmic}
\label{alo1}
\end{algorithm}
%----------------------------

%\subsection{Difference between our approach and meta-learning with pre-training}
\subsection{Difference to meta-learning with pre-training}
The meta-learning with pre-training method typically involves two distinct stages, as illustrated in Figure \ref{fig1}, namely pre-training and meta-training. During the pre-training stage, the model undergoes conventional classification training to acquire convergent feature extractor parameters. Subsequently, in the meta-training stage, the model is retrained using few-shot learning mechanism, leveraging the previously obtained convergent model parameters.
However, employing further optimization within the already convergent model space poses the risk of encountering overfitting issues, as depicted in Figure \ref{fig:dif-measure}. This scenario makes it challenging to achieve additional enhancements in model accuracy. 

In contrast, our proposed approach deviates from this phased training paradigm. Instead, it adopts a strategy that combines classification training with several few-shot learning tasks at each iteration, guiding the parameter updates, as depicted in Figure \ref{fig2}.
To elaborate, the outer loop initially calculates the classification loss for a batch of data, while the inner loop computes the loss for few-shot task. The model parameters are then updated based on both losses %refer to
as in \eqref{e6}. By fully updating the model at each step, our approach mitigates the risk of premature overfitting, ensuring a more robust training process.

% \begin{figure}
% \begin{center}
%   \includegraphics[width=0.9\linewidth]{boost-mt-b.png} 
% \end{center}
%    \caption{The parameter updating procedure of our model. In the outer loop, we calculate the classification loss of one large batch from base classes. In the inner loop, we use the meta-learning method to calculate the loss of tasks and update the model by inner loss and outer loss.}
% \label{fig:svrg_metabaseline}
% \end{figure}

\begin{figure}
\centering
\subfloat[]{\includegraphics[width=0.45\linewidth]{boost-mt-a.png}%
\label{fig1}}
\hfil
\subfloat[]{\includegraphics[width=0.475\linewidth]{boost-mt-b.png}%
\label{fig2}}
\caption{The parameter update procedures of the Meta-Baseline and our model.  In Meta-Baseline, meta-training continues on the model parameters that have been converged in pre-training, as shown in (a). 
In contrast, our model employs an end-to-end training process as illustrated in (b). In the outer loop, we compute the classification loss for a large batch from base classes. In the inner loop, we utilize the meta-learning method to calculate task losses and update the model based on both inner and outer losses.}
\label{fig:svrg_metabaseline}
\end{figure}
